Smarter Cities with Parked Cars as Roadside Units

Real-time monitoring of traffic density, road congestion, public transportation, and parking availability are key to realizing the vision of a smarter city and, with the advent of vehicular networking technologies such as IEEE 802.11p and WAVE, this information can now be gathered directly from the vehicles in an urban area. To act as a backbone to the network of moving vehicles, collecting, aggregating, and disseminating their information, the use of parked cars has been proposed as an alternative to costly deployments of fixed Roadside Units. In this paper, we introduce novel mechanisms for parking vehicles to self-organize and form efficient vehicular support networks that provide widespread coverage to a city. These mechanisms are innovative in their ability to keep the network of parked cars under continuous optimization, in their multi-criteria decision process that can be focused on key network performance metrics, and in their ability to manage the battery usage of each car, rotating roadside unit roles between vehicles as required. We also present the first comprehensive study of the performance of such an approach, via realistic modeling of mobility, parking, and communication, thorough simulations, and an experimental verification of concepts that are key to self-organization. Our analysis brings strong evidence that parked cars can serve as an alternative to fixed roadside units, and organize to form networks that can support smarter transportation and mobility.

==> tables/algoCountCoveredCells.tex <==
%!TEX root = ../advOptJournal.tex
\begin{algorithm}
\DontPrintSemicolon
\KwData{$[\SCM_{\sol_k}]$, $\mathcal{N}_2$}
\KwResult{$\mathrm{cov}_{\sol_k}$: the number of covered cells in $\sol_k$}
$\triangleright$ $\lm_{xy}$ (in an empty $\LM$) are initialized to $0$ \;
$\mathrm{cov}_{\sol_0} \gets 0$ \;
\ForEach{$\SCM_n\in\{\SCM_{\sol_k}, \mathcal{N}_2\}$}{
	\ForEach{$\scm_{n[xy]}\in\SCM_n$}{
		\lIf{$\scm_{n[xy]} > 0$}{$\lm_{xy}\gets{}1$}
	}
}
\ForEach{$\lm_{xy}\in\LM$}{
	\lIf{$\lm_{xy}==1$}{$\mathrm{cov}_{\sol_k} = \mathrm{cov}_{\sol_k} + 1$}
}
\caption{CountCoveredCells\label{alg:bestcovsize}}
\end{algorithm}

==> tables/powerConsumption.tex <==
%!TEX root = ../advOptJournal.tex
\begin{table}[!htbp]
%	\renewcommand{\arraystretch}{1.3}
\small
	\centering
	\caption{Average Power Draw of Major OBU Systems}
	\label{tab:powerConsumption}
\begin{tabular}{@{}ll@{}}
\toprule
Base system                           	& 1.64 W \\
CPU under 100\% load                  	& 0.45 W \\
DSRC transmission at 100\% duty cycle 	& 1.75 W \\
DSRC transmission at 50\% duty cycle  	& 0.75 W \\ 
Powering DSRC radio               		& 2.42 W \\
Powering WiFi radio               		& 0.49 W \\
DSRC reception at 100\% duty cycle		& 0.21 W \\
DSRC reception at 50\% duty cycle 		& 0.10 W \\ 
\bottomrule
\end{tabular}
\end{table}

==> texfigures/annotatedpower.tex <==
%!TEX root = ../advOptJournal.tex
\begin{figure*}[!htbp]
	\centering
	\includegraphics[width=\linewidth]{D0_annotatedPower}
	\caption{Instantanous power demand by an on-board unit performing common tasks.}
	\label{fig:annotatedpower}
\end{figure*}

==> texfigures/histselected.tex <==
%!TEX root = ../advOptJournal.tex
\begin{figure}[!htbp]
	\centering
	% l b r t
	\includegraphics[scale=1.0,trim={262mm 77mm 150mm 144mm},clip,frame]{A2_histograms} \quad
	\includegraphics[scale=1.0,trim={280mm 95mm 132mm 126mm},clip,frame]{A2_histograms} \quad
	\includegraphics[scale=1.0,trim={298mm 95mm 114mm 126mm},clip,frame]{A2_histograms} 
	\label{fig:histselected}
\end{figure}

% \begin{figure}[!htbp]
% 	\centering
% 	% l b r t
% 	\includegraphics[scale=1.0,trim={262mm 77mm 150mm 144mm},clip,frame]{A2_histograms} \quad
% 	\includegraphics[scale=1.0,trim={280mm 95mm 132mm 126mm},clip,frame]{A2_histograms} \quad
% 	\includegraphics[scale=1.0,trim={298mm 95mm 114mm 126mm},clip,frame]{A2_histograms}
% 	\caption{In cells where corner obstructions are present, received signal strength will often exhibit a bimodal distribution.}
% 	\label{fig:histselected}
% \end{figure}

% \begin{figure}[!htbp]
% 	\centering
% 	% l b r t
% 	\includegraphics[scale=1.0,trim={262mm 98mm 150mm 162mm},clip,frame]{A0_histograms} \quad
% 	\includegraphics[scale=1.0,trim={280mm 116mm 132mm 144mm},clip,frame]{A0_histograms} \quad
% 	\includegraphics[scale=1.0,trim={298mm 116mm 114mm 144mm},clip,frame]{A0_histograms}
% 	\caption{In cells where corner obstructions are present, received signal strength will often exhibit a bimodal distribution.}
% 	\label{fig:histselected}
% \end{figure}
